Formation of ultracold triatomic molecules by electric microwave association

A theoretical model is proposed for the formation of ultracold ground-state triatomic molecules in weakly bound energy levels. The process is driven by the electric component of a microwave field, which induces the association of an ultracold atom colliding with an ultracold diatomic molecule. This model is exemplified using $^{39}$K atoms and $^{23}$Na$^{39}$K molecules, both in their ground states, a scenario of experimental relevance. The model assumes that the dynamics of the association are dominated by the long-range van der Waals interaction between $^{39}$K and $^{23}$Na$^{39}$K. The electric microwave association mechanism relies on the intrinsic electric dipole moment of $^{23}$Na$^{39}$K, which drives transitions between its lowest rotational levels ( $j$=0 and $j$=1). The energies of the uppermost triatomic energy levels are computed by numerically solving coupled Schr\"odinger equations using the Mapped Fourier Grid Hamiltonian method. Measurable association rates are derived within the framework of a perturbative approach. This method of electric microwave association provides an alternative to atom-molecule association via magnetic Feshbach resonances for forming ultracold, deeply bound triatomic molecules, and is applicable to a wide range of polar diatomic molecules.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
      system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
